Rethinking the editing of generative adversarial networks: a method to estimate editing vectors based on dimension reduction

While Generative Adversarial Networks (GANs) have recently found applications in image editing, most previous GAN-based image editing methods require largescale datasets with semantic segmentation annotations for training, only provide high level control, or merely interpolate between different images. Previous researchers have proposed EditGAN for high-quality, high-precision semantic image editing with limited semantic annotations by finding `editing vectors'. However, it is noticed that there are many features that are not highly associated with semantics, and EditGAN may fail on them. Based on the orthogonality of latent space observed by EditGAN, we propose a method to estimate editing vectors that do not rely on semantic segmentation nor differentiable feature estimation network. Our method assumes that there is a correlation between the intensity distribution of features and the distribution of hidden vectors, and estimates the relationship between the above distributions by sampling the feature intensity of the image corresponding to several hidden vectors. We modified Linear Discriminant Analysis (LDA) to deal with both binary feature editing and continuous feature editing. We then found that this method has a good effect in processing features such as clothing type and texture, skin color and hair.

==> multiLDA.tex <==
Given a dataset $\mathbf{X}$ with $M$ labels, we can separate the dataset into several groups according to the labels, which is denoted as $\mathbf{X}_i$, where $i \in \{1,...,M\}$. In each group $\mathbf{X}_i$ of size $n_i$, we denote $x_{ij} \in \mathbb{R}^N$ as the data point in this group where $j \in \{1,...,n_i\}$ and $m_{i}$ as the group center, i.e. $m_{i} = \frac{1}{\mathbf{n_i}}\sum_j x_{ij}$. Denote $\Bar{m}$ as the center of the whole dataset $\mathbf{X}$. 

In order to get a good classification result, we need to maximize variance between groups $Var_{bg}$ and minimize variance in groups $Var_{ig}$ after projection. Denote $\mu \in \mathbb{R}^N$ as the projection vector. Hence, we can calculate both two variances. 
\begin{equation}
    \begin{aligned}
        Var_{bg} = \sum_{i=1}^{M}\left[ \mu^T(m_i- \Bar{m})\right]^2 = \mu^T \left(\sum_{i=1}^{M} (m_i-\Bar{m})(m_i-\Bar{m})^T \right)\mu
    \end{aligned}
\end{equation}
\begin{equation}
    Var_{ig} = \sum_{i=1}^{M} \sum_{j=1}^{n_i} \left[\mu^T(x_{ij}-m_i)\right]^2 = \mu^T \left(\sum_{i=1}^{M} \sum_{j=1}^{n_i}(x_{ij}-m_i)(x_{ij}-m_i)^T\right)\mu
\end{equation}
For convenience, we denote $V = \sum_{i=1}^{M} \sum_{j=1}^{n_i}(x_{ij}-m_i)(x_{ij}-m_i)^T$ and $S = \sum_{i=1}^{M} (m_i-\Bar{m})(m_i-\Bar{m})^T$. 

In order to maximize $Var_{bg}$ and minimize $Var_{ig}$ at the same time, we formulate the following optimization problem:
\begin{eqnarray}
    \max_{\mu} \qquad \frac{\mu^T V \mu}{\mu^T S \mu} \label{pre_opt}
\end{eqnarray}
It is trivial to see that \eqref{pre_opt} is equivalent to the following:
\begin{eqnarray}
\begin{aligned}
    \max_{\mu} & \qquad \mu^T V \mu \\
    \mathrm{s.t.} & \qquad \mu^TS\mu = 1.
\end{aligned}
\end{eqnarray}
By applying Lagrange multipliers, we could define the Lagrange function $L$:
\begin{equation}
    L = \mu^T V \mu - \lambda(\mu^TS\mu - 1)
\end{equation}
According to the KKT conditions, we could get the optimal value is the biggest eigenvector $\lambda_1$ of $S^{-1}V$ and the corresponding solution $\mu^*$ is the corresponding eigenvector of $\lambda_1$.

Noting that $S$ may not be invertible, which could block the calculation. We could use some technique to avoid this situation. Denote $\epsilon$ as a small number and $I \in \mathbb{R}^{N\times N}$ as the identity matrix. We add $\epsilon I$ to $S$ to keep the new $S$ invertible.
